Investigating Opportunities to Support Kids' Agency and Well-being: A Review of Kids' Wearables

Wearable devices hold great potential for promoting children's health and well-being. However, research on kids' wearables is sparse and often focuses on their use in the context of parental surveillance. To gain insight into the current landscape of kids' wearables, we surveyed 47 wearable devices marketed for children. We collected rich data on the functionality of these devices and assessed how different features satisfy parents' information needs, and identified opportunities for wearables to support children's needs and interests. We found that many kids' wearables are technologically sophisticated devices that focus on parents' ability to communicate with their children and keep them safe, as well as encourage physical activity and nurture good habits. We discuss how our findings could inform the design of wearables that serve as more than monitoring devices, and instead support children and parents as equal stakeholders, providing implications for kids' agency, long-term development, and overall well-being. Finally, we identify future research efforts related to designing for kids' self-tracking and collaborative tracking with parents.

==> contents/tables/communication_old.tex <==
\begin{table}[]
\begin{tabular}{p{4.2cm}p{7.7cm}r}
%\multicolumn{3}{c}{\textbf{Table 2: Connectedness features}}                                                                                                                                                   
\multicolumn{3}{c}{\textbf{One-way communication}}                                                                                                                                                              
\\ \hline
\textbf{Features} & \textbf{Description} & \textbf{\% Devices (\textit{N} = 47)} 
\\ \hline
One-way haptic feedback              & Parents can send vibrations to device                                                                                          & 4\%                                              \\ \hline
One-way call with auto-pickup        & Children cannot decline calls from parents                                                                                        & 2\%                                              \\ \hline
One-way call without auto-pickup     & Children have option to pickup call from parents                                                                               & 2\%                                              \\ \hline
One-way text message                 & Only parents can send text messages to child                                                                                   & 2\%                                              \\ \hline
\addlinespace[2ex]
\multicolumn{3}{c}{\textbf{Two-way communication}}                                                                                                                                                                       \\ \hline
\textbf{Features} & \textbf{Description} & \textbf{\% Devices (\textit{N} = 47)} 
\\ \hline
Calls                                & Two way calls between parent and child using voice and video                        & 47\%                                             \\ \hline
Messaging                            & Two way messaging between parent and child, such as video, text, and group messages & 34\%                                             \\ \hline
Add/find friends (with the same watch) & Children can add friends with the same device to a contact list                     & 17\%                                             \\ \hline
\end{tabular}
\vspace{1mm}
\caption{An overview of connectedness features, grouped by one-way and two-way communication.}
\vspace{-3mm}
\label{tab:communication}
\end{table}
